MVImgNet: A Large-scale Dataset of Multi-view Images

Being data-driven is one of the most iconic properties of deep learning algorithms. The birth of ImageNet drives a remarkable trend of "learning from large-scale data" in computer vision. Pretraining on ImageNet to obtain rich universal representations has been manifested to benefit various 2D visual tasks, and becomes a standard in 2D vision. However, due to the laborious collection of real-world 3D data, there is yet no generic dataset serving as a counterpart of ImageNet in 3D vision, thus how such a dataset can impact the 3D community is unraveled. To remedy this defect, we introduce MVImgNet, a large-scale dataset of multi-view images, which is highly convenient to gain by shooting videos of real-world objects in human daily life. It contains 6.5 million frames from 219,188 videos crossing objects from 238 classes, with rich annotations of object masks, camera parameters, and point clouds. The multi-view attribute endows our dataset with 3D-aware signals, making it a soft bridge between 2D and 3D vision. We conduct pilot studies for probing the potential of MVImgNet on a variety of 3D and 2D visual tasks, including radiance field reconstruction, multi-view stereo, and view-consistent image understanding, where MVImgNet demonstrates promising performance, remaining lots of possibilities for future explorations. Besides, via dense reconstruction on MVImgNet, a 3D object point cloud dataset is derived, called MVPNet, covering 87,200 samples from 150 categories, with the class label on each point cloud. Experiments show that MVPNet can benefit the real-world 3D object classification while posing new challenges to point cloud understanding. MVImgNet and MVPNet will be publicly available, hoping to inspire the broader vision community.

==> figures/fig_MVP_dist.tex <==
\begin{figure}[t]
    \centering
    \def\svgwidth{\columnwidth}
    \includesvg[inkscapelatex=false]{imgs/haolin_pie8.svg}
    \caption{\textbf{Category distribution of MVPNet}, where the area size of each class denotes its actual data proportion.}
    \label{fig:MVP_dist}
\end{figure}

==> figures/fig_cls_var.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{imgs/cls_var_cat.png}
   \caption{\mt{Some frames sampled from our multi-view videos.}} 
   \label{fig:cls_var}
\end{figure}

==> figures/fig_nerf.tex <==
%\newcommand{\gtfigheight}{0.1\textwidth}
%\newcommand{\resultsheight}{0.12\textwidth}
\newcommand{\gtfigwidth}{0.1\textwidth}
\newcommand{\resultswidth}{0.125\textwidth}

\newcommand{\insertimg}[1]{
  \makecell{
  \includegraphics[width=\resultswidth]{#1} \\
  }
}


\begin{figure*}[t]
	\centering
	\scriptsize
	\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}@{}c@{\,\,}c@{}c@{}c@{}}
		\makecell[c]{
			\includegraphics[trim={0px 0px 0px 0px}, clip, width=\gtfigwidth]{imgs/nerf_comp/ball_457_64526_127116/gt}
			\\
			\textit{Ball}
		}
		& 
		\insertimg{imgs/nerf_comp/ball_457_64526_127116/crop_gt} &
		\insertimg{imgs/nerf_comp/ball_457_64526_127116/crop_IBRNet} &
		\insertimg{imgs/nerf_comp/ball_457_64526_127116/crop_ours} &
		\makecell[c]{
			\includegraphics[trim={0px 0px 0px 0px}, clip, width=\gtfigwidth]{imgs/nerf_comp/bench_415_57112_110099/gt}
			\\
			\textit{Bench}
		}
		&
		\insertimg{imgs/nerf_comp/bench_415_57112_110099/crop_gt} &
		\insertimg{imgs/nerf_comp/bench_415_57112_110099/crop_IBRNet} &
		\insertimg{imgs/nerf_comp/bench_415_57112_110099/crop_ours} \\
		\makecell[c]{
			\includegraphics[trim={0px 0px 0px 0px}, clip, width=\gtfigwidth]{imgs/nerf_comp/book_247_26469_51778/gt}
			\\
			\textit{Book}
		}
		& 
		\insertimg{imgs/nerf_comp/book_247_26469_51778/crop_gt} &
		\insertimg{imgs/nerf_comp/book_247_26469_51778/crop_IBRNet} &
		\insertimg{imgs/nerf_comp/book_247_26469_51778/crop_ours} &
		\makecell[c]{
			\includegraphics[trim={0px 0px 0px 0px}, clip, width=\gtfigwidth]{imgs/nerf_comp/cake_374_42274_84517/gt}
			\\
			\textit{Cake}
		}
		&
		\insertimg{imgs/nerf_comp/cake_374_42274_84517/crop_gt} &
		\insertimg{imgs/nerf_comp/cake_374_42274_84517/crop_IBRNet} &
		\insertimg{imgs/nerf_comp/cake_374_42274_84517/crop_ours} \\
		& Ground Truth  &  Scratch & MVImgNet-pretrained & & Ground Truth & Scratch & MVImgNet-pretrained
	\end{tabular}
	\caption{Qualitative comparison of MVImgNet-pretrained IBRNet~\cite{wang2021ibrnet} model and the train-from-scratch model.}
	\vspace{-0.2cm}
	\label{fig:nerf}
\end{figure*}

==> figures/fig_nerf_sincol.tex <==
%\newcommand{\gtfigheight}{0.1\textwidth}
%\newcommand{\resultsheight}{0.12\textwidth}
\newcommand{\gtfigwidth}{0.2\linewidth}
\newcommand{\resultswidth}{0.25\linewidth}

\newcommand{\insertimg}[1]{
  \makecell{
  \includegraphics[width=\resultswidth]{#1} \\
  }
}


\begin{figure}[t]
	\centering
	\scriptsize
	\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}}
		\makecell[c]{
			\includegraphics[trim={0px 0px 0px 0px}, clip, width=\gtfigwidth]{imgs/nerf_comp/ball_457_64526_127116/gt}
			\\
			\textit{Ball}
		}
		& 
		\insertimg{imgs/nerf_comp/ball_457_64526_127116/crop_gt} &
		\insertimg{imgs/nerf_comp/ball_457_64526_127116/crop_IBRNet} &
		\insertimg{imgs/nerf_comp/ball_457_64526_127116/crop_ours} \\
		\makecell[c]{
			\includegraphics[trim={0px 0px 0px 0px}, clip, width=\gtfigwidth]{imgs/nerf_comp/cake_374_42274_84517/gt}
			\\
			\textit{Cake}
		}
		& 
		\insertimg{imgs/nerf_comp/cake_374_42274_84517/crop_gt} &
		\insertimg{imgs/nerf_comp/cake_374_42274_84517/crop_IBRNet} &
		\insertimg{imgs/nerf_comp/cake_374_42274_84517/crop_ours} \\
		& Ground Truth  &  Scratch & \textbf{MVImgNet-pretrained} 
	\end{tabular}
	\caption{\textbf{NeRF} qualitative comparison of \textbf{MVImgNet-pretrained} IBRNet~\cite{wang2021ibrnet}, CO3D~\cite{co3d}-pretrained IBRNet and the \textbf{train-from-scratch} IBRNet.
	}
	\label{fig:nerf}
 % \vspace{-0.4cm}
\end{figure}

==> figures/fig_pc_pano.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.7\linewidth]{imgs/pointcloud_pano.png}
   \caption{Some dense reconstructed \textbf{3D point clouds} sampled from \textbf{MVPNet}.} 
   \label{fig:mvppano}
\end{figure*}

==> tables/tab_dataset_comp.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c}
    \toprule
    Dataset & Real &\# of samples & \# of categories & 3D-GT\\
    \midrule
    ModelNet~\cite{modelnet}  & \XSolid& 12,311 & 40 & CAD model\\
    ShapeNet~\cite{shapenet} &\XSolid & 52,470 & 55 & CAD model\\
    PASCAL3D ~\cite{pascal3d} & & & &
    CO3D~\cite{co3d} & \Checkmark& 5,625 & 50 & pcl\\
    ScanObjectNN~\cite{scanobjectnn} & \Checkmark& 14,298 & 15 & pcl\\
    MVPNet & \Checkmark& 80,000 & 150& pcl\\
    \bottomrule
    \end{tabular}
    % }
    \caption{\textbf{Comparison between MVPNet and existing datasets} of 3D object point clouds.}
    \label{tab:dataset_comp}
\end{table}

==> tables/tab_scalability.tex <==
\begin{table}[]
    \centering
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
    Method & from scratch& quarter& half& full\\
    \midrule
    PointNet++~\cite{qi2017pointnet++} & 76.50/73.42&77.82/75.98 & 78.11/76.13  &78.76/76.54\\
    CurveNet~\cite{xiang2021walk} & 73.96/69.96 & 73.75/69.86 &75.83/72.48 &78.99/76.59\\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Real-world point cloud classification results} of \textbf{using different amount of data from MVPNet for pretraining}}
    \label{tab:scalability}
\end{table}

==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

